Weighted total variation based convex clustering

Data clustering is a fundamental problem with a wide range of applications. Standard methods, eg the $k$-means method, usually require solving a non-convex optimization problem. Recently, total variation based convex relaxation to the $k$-means model has emerged as an attractive alternative for data clustering. However, the existing results on its exact clustering property, ie, the condition imposed on data so that the method can provably give correct identification of all cluster memberships, is only applicable to very specific data and is also much more restrictive than that of some other methods. This paper aims at the revisit of total variation based convex clustering, by proposing a weighted sum-of-$\ell_1$-norm relating convex model. Its exact clustering property established in this paper, in both deterministic and probabilistic context, is applicable to general data and is much sharper than the existing results. These results provided good insights to advance the research on convex clustering. Moreover, the experiments also demonstrated that the proposed convex model has better empirical performance when be compared to standard clustering methods, and thus it can see its potential in practice.

==> document.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Comparison with related works}
\label{sec:comparison}
First of all, we establish a direct comparison with the result in \cite{zhu2014convex}.
For a pair of $n$-dimensional clusters, denoted by $\CS^{(i)}$ and $\CS^{(j)}$, define their
\emph{intra-class distance} by
\begin{equation}\label{eqn:intradist}
\dist(\CS^{(i)},\CS^{(j)})={\inf}_{x\in \CS^{(i)}, y\in \CS^{(j)}}\|x-y\|_2.
\end{equation}
For a   cluster $\mathcal{S}$, define its
\emph{inner-class distance} (diameter of cluster $\mathcal{S}$) by
\begin{equation}\label{eqn;innerdist}
\dia(\CS)=\sup_{x\neq y\in \CS} \|x-y\|_2.
\end{equation}
Zhu et al. in \cite{zhu2014convex} studied the exact clustering
condition for  $2$-cluster problems via the convex model
\cref{eqn:convex}, and showed  that  two clusters, $\CS^{(0)}$ and $\CS^{(1)}$, can be exactly clustered via \cref{eqn:convex}, provided that
\begin{equation}\label{eqn:zhu}
\dist(\CS^{(0)},\CS^{(1)})>
\max_{k=0,1}\left(1+2\frac{m_{1-k}(m_k-1)}{m_k^2}\right)\dia (\CS^{(k)}),
\end{equation}
where $m_k$ denotes the sample size of the cluster $\CS^{(k)}$.
It can be seen that the low-bound of intra-class distance for exact clustering  increases when the size ratio of two
clusters increases. Even in the optimal setting where two clusters are of same size,
exact clustering condition \eqref{eqn:zhu} requires the intra-class distance at least
three times  of the  inner-class distances.
In terms of  theoretical guarantee of exact clustering, the applicability of model \cref{eqn:convex} is not comparable to that of many popular methods,
e.g., single linkage clustering,  which only requires the intra-class distance larger than the inner-class distances of each cluster.


In this paper, we present a rigorous analysis on exact clustering properties of model \cref{eqn:weightedconvex}.
For any data matrix $A$ whose rows are arbitrarily chosen from one of the $K$ clusters $\mathcal{S}^{(i)}$ ($0\leq i\leq K-1$), we proved that the model \cref{eqn:weightedconvex} will correctly identify the memberships of all rows, if
\begin{equation}\label{eqn:K_sep}
\min_{i\neq j}\dist(\CS^{(i)},\CS^{(j)})>\max_{0\leq i\leq K-1}\dia(\CS^{(i)}),
\end{equation}
and the centers of all clusters are distinct along each dimension. For $2$-cluster setting, it is shown
in \cref{theorem_twobody} that the model \cref{eqn:weightedconvex} can achieve exact clustering for clusters $\CS^{0}$ and $\CS^{1}$, as long as
\begin{equation}
\label{eqn:2_sep}
\dist(\CS^{(0)},\CS^{(1)})>\max\{\dia(\CS^{(0)}),\dia(\CS^{(1)})\}.
\end{equation}
Clearly, in contrast to the existing work on sum-of-$\ell_2$-norm relating convex clustering \cite{zhu2014convex}, 
 Not only, our results are applicable to general $k$-cluster setting ($k\geq 2)$ while \cite{zhu2014convex} is limited to $2$-cluster setting,
 but also our exact clustering condition   is much
less restrictive than that \cite{zhu2014convex} in the sense that ours is independent to cluster size while \cite{zhu2014convex} does.

Indeed, the exact clustering condition \cref{eqn:K_sep} is also less restrict than  many existing  clustering methods, particularly regarding the independence of cluster size and the number of clusters. The result comparison also sheds light on differences between different convex relaxations. 

The exact clustering property for some other convex relaxations of k-means method \cref{eqn:nonconvex} are established in probability context, i.e., the exact clustering with a overwhelming probability. 
We  will apply our exact clustering condition  to some specific distributions on the datasets.  

In \cite{awasthi2015relax,iguchi2015tightness}, the input data matrix $A$ is sampled from the stochastic ball model, see \cref{def:stochastic_ball}.
Denote 
\begin{equation}
\label{eqn:center_distance}
\Delta=\min_{i\neq j} \|\mu_i-\mu_j\|_2
\end{equation}
as the smallest distance between the ball centres. The condition $\cref{eqn:K_sep}$ can be rewritten as 
\begin{equation}
\label{eqn:sep_unitball}
\Delta\geq 4,
\end{equation}
which is sufficient for exact recovery of $K$ clusters in model \cref{eqn:weightedconvex}.

In \cite{awasthi2015relax,iguchi2015tightness}, the authors introduced other kinds of convex relaxation of the $k$-means method: linear programming (LP) relaxation and semidefinite programming (SDP) relaxation.  
The linear programming (LP) relaxation of $k$-means method in \cite{awasthi2015relax} is 
\begin{equation}
\begin{split}
(\text{k-means}\  \text{LP})&\min_{z\in \mathbb{R}^{m\times m}}\sum_{1\leq i,j\leq m}\|A_i-A_j\|_2^2 z_{ij}\\
\text{s.t.}\ &\sum_{1\leq j\leq m}z_{ij}=1,\  z_{ij}\leq z_{ii},\ \sum_{1\leq i\leq m}z_{ii}=K\\
&z_{ij}\in [0,1],\ \text{for}\ \text{all}\ i,j\in [1,...m]\\
\end{split}
\end{equation}
 The result in \cite{awasthi2015relax} showed that the k-means LP succeeds to recover the exact clusters with high probability only in the regime $\Delta\geq 4$. The condition is the same as our exact recovery condition of model \cref{eqn:weightedconvex}. However, the number of points in each cluster should be equal in , which means that the condition in \cite{awasthi2015relax} cannot be applied to the dataset with extremely unbalanced cluster size.
 
 For semidefinite programming (SDP) relaxation, the convex relaxation model becomes 
 \begin{equation}
 \label{eqn: SDP}
 \begin{split}
 (\text{k-means}\ \text{SDP})\ &\max_{X\in \mathbb{R}^{m\times m}} -\text{Tr}(DX)\\
 \text{s.t.}\quad & \text{Tr}(X)=K,\ X\textbf{1}=\textbf{1},\ X\geq 0,\text{and}\  X\succeq 0,\\
 \end{split}
 \end{equation} 
 where $D$ denotes the matrix whose $(i,j)$th entry is $\|A_i-A_j\|_2^2$. 
 
 In \cite{awasthi2015relax}, the authors demonstrated a sufficient condition of exact recovery in the regime 
 \[
 \Delta>2\sqrt{2}(1+\sqrt{1/n}).
 \]
 The condition above is dependent on feature dimension and is weaker than condition $\cref{eqn:sep_unitball}$ when the feature dimension is small.
 
  In \cite{iguchi2015tightness}, the k-means SDP relaxation \cref{eqn: SDP} recovers the planted clusters in stochastic ball model with high probability, provided with \begin{equation}
  \label{eqn:SDP_sep}
 \Delta >2+\frac{K^2}{n}\text{Cond}(\mu),\end{equation} where  
 $\text{Cond}(\mu)=\max_{i\neq j}\|\mu_i-\mu_j\|_2^2\large/\min_{i\neq j}\|\mu_i-\mu_j\|_2^2$. This separation conditions is slightly weaker than the condition \eqref{eqn:sep_unitball} for certain cases. However, when the maximal distance between centers is large and feature dimension is small, i.e. $\text{Cond}(\mu)$ is large while $n$ is small, the condition in \cite{iguchi2015tightness} will be weaker than condition \eqref{eqn:sep_unitball}. Besides, the number of clusters also effects the separation condition on \cref{eqn:SDP_sep}, while our condition \eqref{eqn:sep_unitball} has no constraint on $K$.
 
 Therefore, the center separation conditions in \cite{awasthi2015relax,iguchi2015tightness} are based on feature dimension and sufficient large sampling number $m$. In contrast, the condition \cref{eqn:sep} does not impose any statistical properties of the data, and  the sufficient condition \cref{eqn:sep_unitball} for exact clustering of stochastic ball model is independent of cluster size and number of clusters, which makes it appealing to the data set with unbalanced cluster size or less sufficient number of samples. Meanwhile, the conditions in \cite{awasthi2015relax,iguchi2015tightness} heavily rely on a specific distribution over data-points drawn i.i.d. from disjoint balls of equal radius, while our condition \cref{eqn:sep} does not depend on data distribution and can be applied to more general datasets, such as mixture of Gaussians. 

As the $k$-means method leads to a non-convex problem, the implementations often use multiple initializations to find a good approximation. In this section, we also show that there is such cases where the trick using multiple initializations can not guarantee the success of the Lloyd's algorithm while convex relaxation model \cref{eqn:weightedconvex} recovers the exact clusters.
Considering $3$ balls of unit radius with the centers of the first two are at a distance of $\Delta>4$ and the center of the third ball is far away. Generate the data by sampling $n$ points from each of these balls. Create $l$ copies of this group of $3$ clusters such that each copy is very far from other copies. Such kind of construction meets the recovery condition of model \cref{eqn:weightconvex}. By the same argument as in \cite{awasthi2015relax}, we can see that the Lloyd's algorithm can succeed with probability at most $(1-2/9)^{l}$ in terms of  random initialization. 

\section{Notations}
\label{sec:notation}
Through this paper, we use the following notations and definitions. We use capital letters for matrices, e.g. matrix $A$, calligraphic capital letters for sets, e.g. index set $\mathcal{I}$, bold small letters with a right arrow overset for column vectors, e.g. $\vec{\textbf{a}}\in \mathbb{R}^m$, and small letters for constant, e.g. $r\in \mathbb{R}^+$. Moreover, $A_p$ denotes the $p$th column of $A$, $A_{pq}$ denotes the entry at $p$th row and $q$th column, and $\vec{\bf{a}}_i$ denotes the $i$th element of $\vec{\bf{a}}$. $\|\cdot\|_{F}$ and $\|\cdot\|$ are the Frobenious norm and
the operator norm respectively, $\text{Tr}(\cdot)$ is the trace of
the matrix. For a vector $\vec{\textbf{a}}$, the $\ell_1,\ell_2$ and $\ell_p$ norms are denoted by $\|\vec{\textbf{a}}\|_1$, $\|\vec{\textbf{a}}\|_2$ and $\|\vec{\textbf{a}}\|_p$, respectively.
	
Given a data matrix $A\in\mathbb{R}^{m\times n}$ sampled from $K$ clusters. Assume there are totally $m_i$ rows of $A$ sampled from the set $\mathcal{S}^{(i)}$, with $0\leq i\leq K-1$. Without loss of generality, let $\mathcal{I}^{(k)}=\{m_{k}+1,m_k+2,\dots,m_k+m_{k+1}\}$ denote the indices of sampling in $\mathcal{S}^{(k)}$, respectively.

By the definition of $\mathcal{I}^{(k)}$, we define the index set $\mathcal{P}^{(0)}$ representing  the difference of two rows from the same cluster:
	\begin{equation} \label{eqn:P0}
	\mathcal{P}^{(0)}=\{(i-1)(m-1)+(j-i)\ |\ i,j\in \mathcal{I}^{(k)},\ 0\leq k\leq K-1\},
	\end{equation}
	and the index set 
	\begin{equation}\label{eqn:P1}
	\mathcal{P}^{(1)}=\{(i-1)(m-1)+(j-i)\ \ |\ \ i\in \mathcal{I}^{(k)},\ j\in \mathcal{I}^{(l)},\ k<l\}
	\end{equation} representing the row indexes of $DX$ which correspond to the difference of two rows from different clusters.
	
	Besides, $\sign(x)$ denotes the signum function of a real number $x$:
	\[
	\sign(x)=
	\left\{\begin{array}{ll}
	-1 & \mbox{if} \ x<0,\\
	0 & \mbox{if} \ x=0,\\
	1 & \mbox{if} \ x>0.
	\end{array}
	\right.
	\]


\section{Main results}
\label{sec:result}
Consider $K$ clusters in $\mathbb{R}^{n}$, denoted by $\mathcal{S}^{(k)}, k=0,1,\ldots,K-1$. Let $A\in \mathbb{R}^{m\times n}$ denote the data matrix whose rows are arbitrarily chosen from these $K$ clusters.
\begin{definition}[exact clustering property]
	A matrix $X\in \mathbb{R}^{m\times n}$ is said to have {exact clustering property}, if it satisifies
	\begin{equation}\label{eqn:exact}
	\left\{\begin{array}{ll}
	X_i=X_j, & \text{if}\  A_i, A_j\in \CS^{(k)},\\
	X_i\neq X_j, & \text{otherwise,}
	\end{array}
	\right.
	\end{equation}
	for any  $1\leq i\neq j\leq m$ and $k=0,1,\dots,K-1$.
\end{definition}

Clearly, given  a  matrix $X$ with exact clustering property, one can correctly group the rows of $X$ into $K$ clusters, by putting the rows with same value into one group, i.e., given a data matrix $A$, a convex model will exactly recover the clusters from $A$ if its minimiser has exact clustering property.

Before presenting the main results for the datasets with $K(\geq 2)$ clusters, we first discuss it in the  $2$-cluster setting for illustrating the main idea.
Recall that the model \cref{eqn:weightedconvex} reads
\begin{equation}\label{eqn:weightconvex}
\hat{X}=\operatornamewithlimits{argmin}_X\|A-X\|^2_F\\
+\sum_{i<j}ce^{-r\|A_i-A_{j}\|_2^2}\|X_i-X_j\|_1,
\end{equation}
the following result shows a sufficient condition of model \cref{eqn:weightconvex} for exact clustering.

\begin{theorem}[$2$-cluster]
	\label{theorem_twobody}
	Let $A\in \mathbb{R}^{m\times n}$ be a data matrix whose rows are arbitrarily sampled from two sets $\mathcal{S}^{(0)}, \mathcal{S}^{(1)}\subset \mathbb{R}^{n}$.
	Suppose that $\mathcal{S}^{(0)}$ and $\mathcal{S}^{(1)}$ satisfy the following separation condition:
	\begin{equation}\label{eqn:sep1}
	\dist(\mathcal{S}^{(0)},\mathcal{S}^{(1)})>\max\{\dia(\mathcal{S}^{(0)}), \dia(\mathcal{S}^{(1)})\}.
	\end{equation}
	Then,  there exist some constants $c,r>0$ such that the minimizer $\widehat X$  of \cref{eqn:weightconvex}
	has exact clustering property \cref{eqn:exact}, i.e. for any $1\leq i\neq j\leq m$,
	$$
	\left\{\begin{array}{ll}
	\widehat{X}_i=\widehat{X}_j, & \mbox{if } \{A_i, A_j\}\subset \CS^{(k)} \mbox{ for } 0\leq k\leq 1,\\
	\widehat{X}_i\neq \widehat{X}_j, & \mbox{otherwise.}
	\end{array}
	\right.
	$$
\end{theorem}
\begin{remark}
Clearly, in the $2$-cluster setting,
our exact clustering condition \eqref{eqn:sep1} is much less restrictive than
the condition \cref{eqn:zhu} for model \eqref{eqn:convex}.
\end{remark}
\begin{remark}[Range of feasible parameters for $2$-cluster]
As shown in the proofs of  \cref{theorem_twobody}, the model  \cref{eqn:weightconvex} guarantees exact clustering, if two parameters $c, r$ are chosen such that
	$$
	r\geq \max \limits_{0\leq i\leq 1}{\ln\left({4\frac{m-m_i}{m_i}}\right)}{(d^2-l_i^2)^{-1}},
	$$
	where 
	\[d=\dist(\mathcal{S}^{(0)},\mathcal{S}^{(1)})\quad \text{and}\quad  l_i=\dia{(\mathcal{S}^{(i)})},\]
	and 
	\[
	\underline{\kappa}(r)\leq c\leq \overline{\kappa}(r).
	\]
	The upper bound $\overline{\kappa}(r)$ of $c$ is given by
		\[
		\min_{p\in\mathcal{P}^{(1)}}\left\{\min_{q\in\mathcal{Q}}\frac{2|\tau_q|}{|{m}(\rho-\gamma_p)|},\min_{q\in\mathcal{Q}}\frac{2|\tau_q|}{m\rho}\right\},
		\]
		and the lower bound $\underline{\kappa}(r)$ of $c$ is given by
		\[
		\max_{0\leq i\leq 1,p\in{\mathcal{P}}^{(0)}}\left\{\frac{\epsilon_i\dia(\mathcal{S}^{(i)})}{\gamma_p-\frac{4(m-m_i)}{m_i}\max\limits_{i\in\mathcal{P}^{(1)}}(\gamma_i)}\right\},
		\]
where  $\tau_q=\frac{1}{m_0m_1}\sum_{i\in\mathcal{P}^{(1)}}(DA)_{iq}$,
		$\epsilon_i=\frac{8(m-m_i)(m_i-1)+4m_i^2}{mm_i^2}$, $\mathcal{Q}=\{q|\tau_q\neq 0\}$ and $\rho=\frac{\sum_{i\in\mathcal{P}^{(1)}}\gamma_i}{m_0m_1}$.

From the explicit form of $\overline\kappa(r)$ and $\underline\kappa(r)$, the length of feasible interval $\Delta \kappa(r)=\overline{\kappa}(r)-\underline{\kappa}(r)$ has the property that $\lim_{r\rightarrow +\infty}\Delta \kappa(r)=+\infty$. See more details in \cref{sec:prf of two-cluster}. Thus, the range of proper parameters is wide, as long as $r$ is chosen sufficiently large.
\end{remark}

The results in the $2$-cluster setting cannot be trivially extended to the general $k(\geq$3)-cluster setting. The main difference is that in the setting of more than $2$ clusters, there is a hidden constraint among different clusters. Taking $3$ clusters in one-dimensional as an example, denote $\hat{x}_{i}$ as the mean value of cluster $\mathcal{S}^{(i)}$, for $i=0,1,2$. Considering the mean value difference between clusters as $\hat{y}^{(i,j)}=\hat{x}_{i}-\hat{x}_{j}$, they satisfy 
\begin{equation}\label{eqn:hidconstraint}
{y}^{(0,1)}+{y}^{(1,2)}={y}^{(0,2)}.
\end{equation}
 See \cref{fig:1D3B} for  illustration.
\begin{figure}
	\centering
	% Requires \usepackage{graphicx}
	\includegraphics[height=0.12\textwidth]{./figure/3body.pdf}\\
	\caption{Example: three one-dimensional clusters $\{\mathcal{S}^{(i)}\}_{i=0,1,2}$.}
	\label{fig:1D3B}
\end{figure}

In contrast, there is no constraint \cref{eqn:hidconstraint}  in the $2$-cluster setting. With additional mild conditions on the centers of the clusters, we obtain the similar results for $K(\geq3)$
clusters.
For the case of $K$ clusters, let $m_i$ and $A_c^{(i)}$ denote the size and the mean  value of cluster $\mathcal{S}^{(i)}$, respectively, i.e. $m_i=\sum_{x\in \mathcal{S}^{(i)}}1$ and $A_c^{(i)}=\frac{1}{m_i}\sum_{x\in \mathcal{S}^{(i)}}x$, then the exact clustering condition to cluster $K$ sets  is established in the following theorem.

\begin{theorem}[$K$-cluster]
	\label{theorem1} 
	Let $A\in \mathbb{R}^{m\times n}$ be a data matrix whose rows are arbitrarily sampled from $K$ sets $\{\mathcal{S}^{(i)}\}_{i=0}^{K-1}\subset \mathbb{R}^{n}$. Suppose that  the cluster means $\{A^{(i)}_c\}_{i=0}^{K-1}$ are distinct in all dimensions, i.e. $(A^{(i)}_c)_p\neq (A^{(j)}_c)_p$ for all $1\leq p\leq n$ and $0\leq i<j\leq K-1$. Suppose that $\{\mathcal{S}^{(i)}\}_{i=0}^{K-1}$ satisfy the following separation condition:
	\begin{equation}\label{eqn:sep}
	\min_{i\neq j}\dist(\mathcal{S}^{(i)},\mathcal{S}^{(j)})>\max_{0\leq k\leq K-1}\dia (\mathcal{S}^{(k)}).
	\end{equation}
	Then,  there exist  $c,r>0$ such that the minimizer $\widehat X$  of \cref{eqn:weightconvex} has exact clustering property \cref{eqn:exact}.\end{theorem}

\begin{remark}
We believe that with more delicate tools, the distinct assumption of cluster centres can be omitted. Whether this condition can be removed is left
to the interested readers.
\end{remark}

\begin{remark}[Range of feasible parameters]\label{remark1} As shown in the proofs of  \cref{theorem1}, the model  \cref{eqn:weightconvex} guarantees exact clustering, if two parameters $c, r$ are chosen such that
	$$
	r\geq \max \limits_{0\leq i\leq K-1}{\ln\left({4\frac{m-m_i}{m_i}}\right)}{(d^2-l_i^2)^{-1}},
	$$
	where 
	\[d=\max_{i\neq j}\dist(\mathcal{S}^{(i)},\mathcal{S}^{(j)})\quad \text{and}\quad  l_i=\dia{(\mathcal{S}^{(i)})},\]
	and 
	\[
	\underline{\kappa}'(r)\leq c\leq \overline{\kappa}'(r).
	\]
	The upper and lower bound of $c$ is similar as $2$-cluster case, where 
		\[
		\overline{\kappa}'(r)=\min_{k<l,1\leq q\leq n}\left\{\frac{|\tau^{k,l}_q|}{3m\max\limits_{j\in\mathcal{P}^{(1)}}(\gamma_j)}\right\}
		\]
		and
		\[
		\underline{\kappa}'(r)=\max_{0\leq i\leq K-1,p\in \mathcal{P}^{(0)}}\left\{\frac{\epsilon_i\dia(\mathcal{S}^{(i)})}{\gamma_p-\frac{4(m-m_i)}{m_i}\max\limits_{j\in \mathcal{P}^{(1)}}(\gamma_j)}\right\}
		\]
				
		It is also easy to show that the feasible interval of $c$, $[\underline{\kappa}'(r),\overline{\kappa}'(r)]$ has the property that $\lim_{r\rightarrow +\infty}\overline{\kappa}'(r)-\underline{\kappa}'(r)=+\infty$; see more details in \cref{sec:prf of three-cluster}. 
\end{remark}

The condition in \cref{theorem1} can be applied to specific distributions on data matrix $A$. For example, the dataset is drawn from stochastic ball model as below.
\begin{definition}[$(\mathcal{D},\mu, m)$-stochastic ball model]
\label{def:stochastic_ball}
Let $\{\mu_i\}_{i=1}^k$ be ball centers in $\mathbb{R}^n$. For each $i$, draw i.i.d. vectors $\{r_{i,j}\}_{j=1}^{m/k}$ from some rotation-invariant distribution $\mathcal{D}$ supported on the unit ball. The points from cluster $i$ are then taken to be $x_{i,j}=r_{i,j}+\mu_{i}$.
\end{definition}

\begin{theorem}
Let $A\in \mathbb{R}^{m\times n}$ be a data matrix drawn from stochastic ball model. Suppose that the ball centers $\mu_i(0\leq i\leq K-1)$ satisfy the separation condition $\min_{i\neq j}\|\mu_i-\mu_j\|\geq 4$, there exist  $c,r>0$ such that the minimizer $\widehat X$  of \cref{eqn:weightconvex} has exact clustering property \cref{eqn:exact}.\end{theorem}
\begin{proof}
Since the marginal distribution of $r_{i,j}$ in each dimension is continuous with non-zero variance, the sample means inside each cluster  are distinct with probability $1$ and the sufficient condition on exact recovery of model \cref{eqn:weightconvex} becomes $\min_{i\neq j}\|\mu_i-\mu_j\|\geq 4$.
\end{proof}

This condition meets the sharp recovery condition of $k$-means LP relaxation in \cite[Theorem 9]{awasthi2015relax}. However, the condition \cref{eqn:sep} requires no assumption on sample size and distribution shape as in \cite{awasthi2015relax}, which heavily depends on equal radii of clusters. Therefore, the condition \cref{eqn:sep} can be  applied to more general distributions besides stochastic ball model, such as mixture of Gaussian. 

\begin{definition}[$(\omega, \mu,\Sigma)$-mixture of Gaussian model]
A mixture of $K$ Gaussian distributions is a distribution in which each sample is drawn from $\mathcal{N}(\mu_{i},\Sigma_{i})$
with probability $\omega_{i}$, where $\sum_i \omega_{i}=1$. 
\end{definition}

Now we apply the recovery condition on mixture of Gaussian model. 
\begin{theorem}
\label{thm:GaussianMixture}
Let $A\in \mathbb{R}^{m\times n}$ be a data matrix whose rows are arbitrarily sampled from mixture of $(\omega, \mu,\Sigma)$-mixture of Gaussian model with $\mu_i(0\leq i\leq K-1)$ distinct in each dimension. Suppose the separation condition is 
\begin{eqnarray*}
\min_{i\neq j}\|\mu_{i}-\mu_{j}\|_{2} & > & \max_{i\neq j}\left(\|\Sigma_{k,l}\|^{\frac{1}{2}}\sqrt{12\log m}+{(12\log m)}^{1/4}\|\Sigma_{k,l}\|_{F}^{1/2}\right)\\
 &  & +{\max}_{i}\sqrt{\mbox{\text{Tr}}(\Sigma_{i})+\|\Sigma_{i}\|_{F}\sqrt{12\log m}+6\|\Sigma_{i}\|\log m},
\end{eqnarray*}
where $\Sigma_{i,j}=\Sigma_{i}+\Sigma_{j}$.
Then there exist some constants $c,r>0$ such that the minimizer $\widehat{X}$
of \cref{eqn:weightconvex} has exact clustering property
with probability larger than $1-3/m$.
\end{theorem}
\begin{remark}
Denote $\sigma_{\max}=\max_i\|\Sigma_i\|^{1/2}$. The separation condition on exact recovery of mixture of $K$ spherical Gaussian distribution becomes $\Omega(\sigma_{\max}\sqrt{n})$. 

In order to eliminate the effect of dimension $n$, partition the sample matrix $A$ uniformly into two submatrices $A_1\in \mathbb{R}^{m/2\times n}$ and $A_2\in \mathbb{R}^{m/2\times n}$. Apply weighted convex model \cref{eqn:weightconvex} to $P_{A_1}(A_2)$ and $P_{A_2}(A_1)$, where $P_X$ is a rank-$K$ projection of matrix $X$, i.e. for any other matrix $Y$ of rank at most $K$, we have $\|X-P_XX\|\leq \|X-Y\|$. By the similar arguments as in \cite{AW05}, the clusters can be recovered with high probability provided with the separation condition $\Omega(\sigma_{\max}\frac{1}{\sqrt{\omega_{\min}}}+\sqrt{K\log m})$ and $\omega_{\min}=\min_i \omega_k$. The condition meets the best separation condition of Gaussian mixture model in literature, see \cite{AR2010,AS12}.
\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:experiments}
Our theoretical analysis showed that the model \cref{eqn:weightconvex} can exactly cluster the dataset, provided that the clusters satisfy certain separation condition. As a paper focuses on theoretical studies of convex clustering, The experiments done in this section is more for understanding the behavior of model \cref{eqn:weightconvex}, not for extensive performance evaluation.

\subsection{Implementation and settings}
The problem \cref{eqn:weightconvex} is a strictly convex problem with at most one local minimiser which is also global minimizer. There are many  efficient numerical solvers for solve \cref{eqn:weightconvex}, e.g. the ADMM method \cite{chi2014convex} and the AMA method~\cite{chi2014splitting}.
In this paper, we use the ADMM method to solve \cref{eqn:weightconvex}. Define the augmented lagrangian function as
\[
L_\nu(X,Z,\Lambda)=\frac{1}{2}\|A-X\|_F^2+c\sum_{l\in\varepsilon}\omega_{l}\|Z_{l}\|_1+\\
\sum_{l\in \varepsilon}\langle\Lambda_l,Z_l-X_{l_1}+X_{l_2}\rangle+\frac{\nu}{2}\sum_{l\in\varepsilon}\|Z_{l}-X_{l_1}+X_{l_2}\|^2_2,
\]
where $l=(l_1,l_2)$ with $l_1<l_2$, and $\varepsilon=\{l=(l_1,l_2):\omega_l>0\}$ is the index set corresponding to non-zero weights\footnote{For efficiency, the implementation only uses weights on the distances of each points and  its $k(=5)$ nearest neighbors.}.
See \cref{alg:admm} for the outline of the algorithm. 
\begin{algorithm}
\caption{The ADMM method}
\label{alg:admm}
\begin{algorithmic}
\STATE {\bfseries Input:} data $A$, regularization $c>0$, weights $\{\omega_{i,j}\}>0$.
					\STATE Initialize $X^{0}=\mathbf{0}, \Gamma^0=\mathbf{0}, Z^0=\mathbf{0}$, $k=0$.
					\STATE Set positive tuning constant $\nu>0$.
					\REPEAT
					\STATE $X^{k+1}=\arg\min_{X}L_\nu(X,Z^k,\Lambda^k)$
					\STATE $Z^{k+1}=\arg\min_{Z}L_\nu(X^{k+1},Z,\Lambda^k)$
					\STATE $\Lambda_{l}^{k+1}= \Lambda^{k}_{l}+\nu(V_{l}-X^{k+1}_{l_1}+X^{k+1}_{l_2})$
					\STATE $k=k+1$
					\UNTIL{$\|X^{k}-X^{k-1}\|_2\leq 10^{-4}$ is satisfied}
					\STATE {\bfseries Return:} $X$ and $Z$
\end{algorithmic}
\end{algorithm}
The algorithm stops when iteration increment  is less than $10^{-4}$.
Once we obtain the solution $\widehat X$ to \cref{eqn:weightconvex} via  \cref{alg:admm}, the clusters are constructed using $\widehat X$ as the replacements of the original ones.
Two observations, $\widehat X_i,\widehat X_j$, belong to the same cluster, as long as  $\|\widehat X_i-\widehat X_j\|_2$ is below a pre-defined threshold (e.g. $10^{-8}$).  As the number of clusters monotonically decreases when the value of regularization parameter $c$ increases  \cite{hocking2011clusterpath}, the number of the clusters is set by using different values of  $c$.

\subsection{Experimental evaluation on synthesized data}
In this section, we would like to evaluate the practical performance of the model \cref{eqn:weightconvex} when being applied on the synthesized datasets that do not
satisfy the conditions imposed in \cref{theorem_twobody} and \cref{theorem1}. As model \cref{eqn:weightconvex} can be viewed
as a convex relaxation of the $k$-means method, we focus on the comparison between the model \cref{eqn:weightconvex} and  two popular  implementations
of the $k$-means method, namely Lloyd's algorithm and \emph{$k$-means$++$}.

\noindent{\bf Clustering mixture of Gaussian}. Dataset of Mixture of Gaussian  is generated by randomly sampling several multivariate normal distributions~(MVN)  $\mathcal{N}(\mu_{i},\sigma^2 I_{n\times n})$, where  $\mu_i$ denotes the mean and $\sigma^2$ denotes the variance. In this experiments, {the dimension of points $n$ is $100$ and the dataset size $m$ is $30$.} Three clusters  corresponding to different distributions with the same cluster size
are generated with $\vec{\mu}_1=0\vec{\bf1}_n$, $\mu_2= 3\vec{\bf1}_n$, $\mu_3= -3 \vec{\bf1}_n$,
where $\vec{\bf1}_n$ denotes the all-ones vector. Two values of variance are tested: $\sigma=1,2$.
The parameter $r$ is set to $r=0.02(2\sigma^2+5\sigma)$. See  \cref{fig:gaussian} for the average Rand index over $100$ runs.
It can be seen that model \cref{eqn:weightconvex} are slightly better in terms of accuracy and noticeably more stable than two $k$-means algorithms.

\begin{figure}
	\centering
	\subfloat[$\sigma=1$]{\label{fig:circle_input}{\includegraphics[width=0.25\textwidth]{./figure/gaussian1.pdf}}}
	\subfloat[$\sigma=2$]{\label{fig:circle_kmeans}{\includegraphics[width=0.25\textwidth]{./figure/gaussian2.pdf}}}
	\caption{Comparison of average Rand index of different methods for clustering mixture of Gaussians over 200 runs. The correspondence
			between plot and method is: Model \cref{eqn:weightconvex}~({\protect\hwplotA}), Lloyd's algorithm~({\protect\hwplotH}), $k$-means++~({\protect\hwplotG}).}
	\label{fig:gaussian}
\end{figure}

\noindent{\bf Clustering non-convex clusters}.\quad
In this experiment, we illustrate the clustering performance on a classic two-body non-convex clusters: two embedded circle clusters~\cite{ng2001spectral}. See \cref{fig:results_circle}(a) for the visualization of such two clusters. It is  known  that the
$k$-means methods are not effective on such a dataset, as it is about minimizing the cluster variances (see e.g. \cite{xu2005survey}.
The dataset is generated as follows.
One cluster (blue points) is given by  randomly sampling $250$ points from a $2$-dimensional  MVN $\mathcal{N}(0,I_{2\times 2})$ under Cartesian coordinate system. The other cluster (red
points) is generated by  randomly sampling $250$ points under polar coordinate system, in which radials follow normal distribution $\mathcal{N}(5,0.25^2)$ and angulars follow uniform distribution $\mathcal{U}(0,2\pi)$.
	
As the $k$-means method is sensitive to initialization, the mean and standard deviation~(SD) of the two $k$-means methods are reported over 100 randomly chosen initializations.    In the experiment, we repeated $k$-means algorithm $100$ times, and calculated the mean and standard deviation~(SD) of all Rand index. See \cref{tab:example} for the comparisons among three methods, and see \cref{fig:results_circle} for the illustration of one instance. The result of model \cref{eqn:weightconvex} is much better than that of two $k$-means algorithms.

\begin{table}
	\caption{\label{tab:example}Rand indexes on clustering non-convex clusters }
	\centering
	\begin{tabular}{|l|*{5}{c|}}\hline
			Method & Lloyd's alg. & $k$-means++ & Model \cref{eqn:weightconvex} \\ \hline
			Mean & 0.517 &0.491& 0.996 \\ \hline
			SD & 0.012 & 0.010 & { 0}  \\ \hline
	\end{tabular}
\end{table}

\begin{figure}
		\centering
		\subfloat[input]{{\includegraphics[width=0.23\textwidth]{./figure/s_input.pdf}}}
		\subfloat[Lloyd's algorithm]{{\includegraphics[width=0.23\textwidth]{./figure/s_kmeans.pdf}}}
		\subfloat[$k$-means++]{{\includegraphics[width=0.23\textwidth]{./figure/s_kmeanspp.pdf}}}
		\subfloat[model \cref{eqn:weightconvex}]{{\includegraphics[width=0.23\textwidth]{./figure/s_ours.pdf}}}
		\caption{Illustrations of clustering non-convex clusters.}
		\label{fig:results_circle}
\end{figure}

\subsection{Experimental evaluation on real data}
In this section, we compared the clustering performance of Model \cref{eqn:weightconvex} with several other methods on  several real data sets. The methods for comparison include two $k$-means algorithm: (1) Lloyd' $k$-means algorithm, (2) $k$-means++, and two hierarchical algorithms: (3) hierarchical single linkage (HC(Sin)), and (4) hierarchical average linkage (HC(Ave)). 
Through the experiments, the so-called \emph{Rand} index is used to evaluate clustering performance; see ~\cite{hubert1985comparing} for more details. It ranges between $0$ and $1$, and larger Rand index  implies better agreement with the true clusters.
The results from Model \cref{eqn:weightconvex} and two linkage methods
are reported from a single pass, and the results from two $k$-means algorithms are reported by taking the average of the outcomes over $100$ tests (each test takes the largest Rand index over $10$ randomly chosen initializations).
%The parameters of all methods are rigorously tuned up for optimal performance.

Four datasets, from  UCI machine learning repository~\cite{Lichman:2013,martinez1998ar} are tested in the experiments, including (1) "Iris": 3 clusters with
average  50 points in $\mathbb{R}^4$  each;
(2) "AR face": 2 clusters with average 350 points in $\mathbb{R}^{300}$ each;
(3) "Libras movement": 15 clusters with average 24 points in $\mathbb{R}^{90}$ each;
(4) "Leaf": 36 clusters with average 10 points in $\mathbb{R}^{14}$ each.

See \cref{fig:results_iris} for the comparison of Rand indexes of the five methods. It can be seen that, in general, Model \cref{eqn:weightconvex} is the top performer among all compared methods, and its performance is consistent on different datasets with different characters.
Particularly, it significantly outperforms the others on AR dataset, which has much larger cluster size and  much higher dimension than the others.
It indicates that the convex relaxation \cref{eqn:weightconvex} of $k$-means method  has its advantages when processing high-dimensional dataset with large cluster size, which is known to be challenging for $k$-means algorithms (see e.g \cite{garcia1999robustness}).
 
 \begin{figure}
	\centering
	\subfloat[Iris]{{\includegraphics[width=0.25\textwidth,height=0.16\textwidth]{./figure/iris_output.pdf}}}
	\subfloat[AR face]{{\includegraphics[width=0.25\textwidth,height=0.16\textwidth]{./figure/AR_output.pdf}}}
	\subfloat[Libras Movement]{{\includegraphics[width=0.25\textwidth,height=0.16\textwidth]{./figure/LM_output.pdf}}}
	\subfloat[Leafs]{{\includegraphics[width=0.25\textwidth,height=0.16\textwidth]{./figure/leafs_output.pdf}}}
	\caption{Comparison of Rand indexes among different methods on different real data sets.  The correspondence between plot and method is: Model \cref{eqn:weightconvex}~({\protect\hwplotA}), Lloyd's alg.~({\protect\hwplotF}), $k$-means++~({\protect\hwplotC}), HC(Sin)~({\protect\hwplotE}) and HC(Ave)~({\protect\hwplotB}).
	}
	\label{fig:results_iris}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
\label{sec:conclusion}
 This paper presented theoretical analysis of a weighted sum-of-$\ell_1$-norm based convex relaxation model to
the $k$-means method. While existing theoretical analysis  in \cite{zhu2014convex} for convex clustering is limited
to two-cluster problem,
our results are applicable to the problem with arbitrarily number of clusters. Also for two-cluster problem, our results impose
much less restrictive exact clustering
condition than existing ones. Actually, the exact clustering condition for $\ell_1$ convex clustering can be less restrict
than that for the well established Lloyd's $k$-means algorithm in the deterministic sense. Besides, since the recovery condition is independent of cluster size and number of clusters, it benefits a lot when applying to mixture of distributions with unbalanced cluster size or dataset with less sufficient number of samples.  The experiments on real datasets also showed better performance of the proposed convex model over some often seen methods.
The studies presented in this paper provide important insights and solid theoretical foundations for further development and studies of  novel convex clustering methods.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibliographystyle{siamplain}
\bibliography{references}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\appendix\label{appendix}
\section{Proof of \cref{theorem_twobody,theorem1}}
The proofs of \cref{theorem_twobody,theorem1} both take three main steps: (1) we derive an equivalent optimization problem of Model \cref{eqn:weightconvex} which is easier to be analysed owing to the variables separation inside $\ell_1$ norm; (2) the dual problem of the optimization is studied by constructing a dual pair for $K=2$ and $K\geq 3$ separately such that the minimizer of the optimization problem has some special properties; (3) based on the special properties derived in the previous step, we prove that  the minimizer of \cref{eqn:weightconvex} has exact clustering property.

	\subsection{Model equivalence and dual problem}
	Before proceeding, we  consider the column-centered version of $A$, denoted by $\tilde{A}$, which is defined as
	\begin{equation}
	\label{eqn:center}
	\tilde{A}=A-C,
	\end{equation}
	where $j$th column of $C$ is a constant vector with value $\frac{1}{m}\sum_{i=1}^mA_{ij}$. It can be seen that the mean of each column of $\tilde A$ is zero.
	
	 First of all, we prove that  Model \cref{eqn:weightconvex} taking $A$ as input is equivalent to Model \cref{eqn:weightconvex} taking $\tilde A$.
\begin{lemma}
		\label{thm:lemma1}
		Let $A\in \mathbb{R}^{m\times n}$ be a data matrix whose rows are arbitrarily sampled from $K$ sets $\mathcal{S}^{(k)}$ ($0\leq k\leq K-1$).
		Let $\tilde A$ denote its column-centered version defined by \eqref{eqn:center}. Then  the minimizer of the model \cref{eqn:weightconvex} has exact clustering property if and only if
		the minimizer of the following optimization problem 		\begin{equation}
		\label{eqn:eq1}
		\min_{\tilde{X}}\|\tilde{A}-\tilde{X}\|^2_F+\sum_{j=2}^m\sum_{i<j}ce^{-r\|\tilde{A}_i-\tilde{A}_j\|_2^2}\|\tilde{X}_i-\tilde{X}_j\|_1
		\end{equation}
		also has exact clustering property.
	\end{lemma}

\begin{proof}
		Suppose $\widehat{\tilde{X}}$ is the minimizer of Problem~\eqref{eqn:eq1}, then for any $X\in\mathbb{R}^{m\times n}$, we have
		\begin{equation*}
		\label{eqn:proof1}
		\begin{split}
		&\|A-X\|^2_F+\sum_{i<j}ce^{-r\|A_i-A_{j}\|_2^2}\|X_i-X_j\|_1\\
		=&\|A-C-(X-C)\|^2_F+\sum_{j=2}^m\sum_{i<j}ce^{-r\|A_i-C_i-(A_j-C_j)\|_2^2}\|X_i-C_i-(X_j-C_j)\|_1\\
		=&\|\tilde{A}-(X-C)\|^2_F+\sum_{j=2}^m\sum_{i<j}ce^{-r\|\tilde{A}_i-\tilde{A}_j\|_2^2}\|X_i-C_i-(X_j-C_j)\|_1\\
		\geq &\|\tilde{A}-\widehat{\tilde{X}}\|^2_F+\sum_{j=2}^m\sum_{i<j}ce^{-r\|\tilde{A}_i-\tilde{A}_{j}\|_2^2}\|\widehat{\tilde{X}}_i-\widehat{\tilde{X}}_j\|_1\\
		=&\|A-(\widehat{\tilde{X}}+C)\|^2_F+\sum_{j=2}^m\sum_{i<j}ce^{-r\|A_i-A_{j}\|_2^2}\|(\widehat{\tilde{X}}_i+C_i)-(\widehat{\tilde{X}}_j+C_j)\|_1.\\
		\end{split}
		\end{equation*}
		Thus, we have $\widehat{\tilde{X}}+C$ as the minimizer of Problem \cref{eqn:weightconvex}. Similarly, if $\hat{X}$ is a minimizer of Problem \cref{eqn:weightconvex}, then $\hat{X}-C$ is the minimizer of Problem \cref{eqn:eq1}.
		Furthermore, suppose $\widehat{\tilde{X}}$ is the minimizer of Problem~\eqref{eqn:eq1}, and it has exact clustering property, then $\widehat{\tilde{X}}_i-\widehat{\tilde{X}}_j=\widehat{\tilde{X}}_i-C_i-(\widehat{\tilde{X}}_j-C_j)$ implies that the minimizer of Problem \cref{eqn:weightconvex} has exact clustering property as well. Similarly, if the minimizer of Problem \cref{eqn:weightconvex} has exact clustering property, then  the minimizer of Problem \cref{eqn:eq1} also has exact clustering property.
	\end{proof}
Therefore, in the remaining of this paper, we will assume that $A$ is column-centred such that the mean of each column of $A$ is zero.

Now we introduce the total difference operator for notation simplicity. 
\begin{definition}[total difference operator]
	\label{def:total}
	Let $G^i=(\textbf{0}_{(i-1)\times(m-i)},\vec{\textbf{1}}_{(i-1)\times 1}, -I_{(i-1)\times(i-1)})$. The total difference operator of order $m$ is defined by
	$$D^m=[(G^{m})^T, (G^{m-1})^T,\dots, (G^2)^T]^T.$$
	Let \[\mathcal{D}=\{D^mX\ |\ X\in \mathbb{R}^{m\times n}\},\]
	 $D^m$ is a linear operator from $\mathbb{R}^{m\times n}$ to $\mathcal{D}$. Moreover, for any $Y\in R^{\binom{m}{2}\times m}$, $Y$ belongs to $\mathcal{D}$ if and only if $HY=0$, where $H=(D^{m-1},I)$.
\end{definition}
\noindent For simplicity,  we take $D=D^m$ unless otherwise stated, and for convenience, set $B=DA$. Using the same arguments as  \cite[Lemma 1, Lemma 2]{zhu2014convex}, we have
\begin{lemma}
	\label{thm:lemma2}
	Given any column centered-matrix $A$, $\hat{X}$ is minimizer of Problem \cref{eqn:weightconvex}, if and only if $D\hat{X}$ is the minimizer of the following problem,
	\begin{equation}
	\label{formula5}
	\hat{Y}=\argmin_{Y\in {\mathcal{D}}}\frac{1}{m}\|B-Y\|_F^2+c\sum_{i=1}^{{ m \choose 2}}\gamma_{i}\|Y_i\|_1,
	\end{equation}
	where $\gamma_i=\exp(-r\|(DA)_i\|_2^2) $, and $\mathcal{D}$ is the range space of $D$  defined by $\mathcal{D}=\{D X\ |\ X\in \mathbb{R}^{m\times n}\}$.
\end{lemma}

The problem \cref{eqn:weightconvex} is now simplified as the entries in sum-of-$\ell_1$-norm separable. To tackle the technical challenges  raised by  the introduced constraint $Y \in \mathcal{D}$,
we consider the dual problem of \cref{formula5}. By standard arguments in convex analysis \cite[Page 301]{bertsekas2009convex}, The variable pair $\{\hat{Y},\hat{\Lambda}\}$ is an optimal primal-dual pair if and only if
\begin{equation}\label{eqn:dual}
\hat{Y_i}=\operatornamewithlimits{argmin}_{Y_i^T\in \mathbb{R}^n}\frac{1}{m}\|B_i-Y_i\|_2^2+c\gamma_i\|Y_i\|_1-Y_i\Lambda_i^T,
\end{equation}
subject to $Y\in \mathcal{D},\ \Lambda^T\in \mathcal{D}^\perp$, where $ \mathcal{D}^\perp$ denotes the orthgonal complement of $\mathcal{D}$.
Hence, to prove $\hat{X}$ of having exact clustering property, it suffices to find some dual parameter $\widehat{\Lambda}^T \in \mathcal{D}^\perp$, such that the corresponding primal minimizer $\hat{Y}\in \mathcal{D}$  has the following form,
\begin{equation}
\label{eqn:solutionform}
\hat{Y}_{p}=
\left\{ \begin{array}{l}
\vec{\textbf{0}},\ \ \ \ \ \makebox{if}\ p\in\mathcal{P}^{(0)},\\
\vec{\textbf{e}}^{k,l},\ \ \makebox{if}\ p\in\mathcal{P}^{(k,l)},
\end{array} \right.
\end{equation}
where $(\vec{\textbf{e}}^{k,l})^T\in \mathbb{R}^n$ is some non-zero constant vector. The index set $\mathcal{P}^{(0)}$ is defined in \cref{eqn:P0} and
\begin{equation}
\label{eqn:Pkl}\mathcal{P}^{(k,l)}=\{(i-1)(m-1)+(j-i)\ |\  i\in \mathcal{I}^{(k)},\ j\in \mathcal{I}^{(l)}\}
\end{equation} represents the row indexes of $DX$ which  are corresponding to the differences of two rows from different clusters $\mathcal{S}^{(k)}$ and $\mathcal{S}^{(l)}$, where $0\leq k<l\leq K-1$. $\mathcal{P}^{(1)}=\cup_{i<j}\mathcal{P}^{(i,j)}$ defined in \cref{eqn:P1} is
the index set of all differences from distinct clusters.

\subsection{Proof of \cref{theorem_twobody}}
\label{sec:prf of two-cluster}
First of all, we show some sufficient condition for primal-dual solver.
\begin{theorem}[sufficient condition for $2$-cluster]
\label{thm:suf_two}
 Assume $c,r\in \mathbb{R}^+$ and $\widehat{\Lambda}^T\in \mathcal{D}^\perp$.  $\vec{\textbf{e}}^T\in \mathbb{R}^n$ is some nonzero column vector. $\mathcal{P}^{(0)}$ and $\mathcal{P}^{(1)}$ are defined in \cref{eqn:P0} and \cref{eqn:P1}.
 
	Suppose for $p\in\mathcal{P}^{(1)}$, $\hat\Lambda_{pq}$ satisfies
	\begin{subequations}
	\begin{align}
	&c\gamma_{p}\leq \frac{2}{m}\left|B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq}\right|,\label{eqn:cond_two10}\\
	&\left(B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq}\right)-\frac{mc\gamma_p}{2}\sign\left(B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq}\right)=\vec{\textbf{e}}_q,\label{eqn:cond_two11}
	\end{align}
	\end{subequations}
		
		 and for $p\in\mathcal{P}^{(0)}$, we have
		\begin{equation}
		\label{eqn:cond_two2}
		c\gamma_p>\frac{2}{m}\left|B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq}\right|,
		\end{equation}
$\widehat{\Lambda}$ is the optimal dual variable in \cref{eqn:dual}, and $\hat{Y}$ can be derived respectively. Together with the fact that $\widehat{Y}=D\widehat{X}$, $\widehat{X}$ satisfies the exact clustering property.
\end{theorem}
\begin{proof}
If $\widehat{\Lambda}$ is  the optimal dual variable in \cref{eqn:dual}, the optimal primal variable $\widehat{Y}$ can be derived as 
\begin{equation}\label{eqn:proof2}
	\widehat{Y}_{pq}=\left(B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq}\right)-\frac{mc \gamma_{p}}{2}\sign\left(B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq}\right),
	\end{equation}
	if $c\gamma_{p}\leq \frac{2}{m}|B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq}|$ and $\widehat{Y}_{pq}=0$ otherwise, for  $p=1,\dots,\binom{m}{2}$ and  $q=1,\dots,n$.

By the conditions \cref{eqn:cond_two10,eqn:cond_two10,eqn:cond_two11,eqn:cond_two2},we can see that 
\begin{equation}
	\label{eqn:solutionform_two}
	\widehat{Y}_{p}=
	\left\{ \begin{array}{l}
	\vec{\textbf{0}},\ \ \mbox{if}\ p\in\mathcal{P}^{(0)},\\
	\vec{\textbf{e}},\ \ \mbox{if}\ p\in\mathcal{P}^{(1)},
	\end{array} \right.
	\end{equation}
which meets the primal minimizer form in \cref{eqn:solutionform}. Therefore, $(\widehat{Y},\widehat{\Lambda})$ is the optimal primal-dual pair in \cref{eqn:dual}.
\end{proof}

Under the sufficient condition in \cref{thm:suf_two}, we have $\widehat{X}$ has exact clustering property with
	\[\widehat{X}_{i,j}=
	\left\{ \begin{array}{l}
	\frac{m_1}{m_0+m_1}\vec{\textbf{e}}_j, \quad i\in\mathcal{I}^{(0)},\\
	\frac{-m_0}{m_0+m_1}\vec{\textbf{e}}_j, \quad i\in\mathcal{I}^{(1)}.
	\end{array} \right.
	\]

We explicitly construct the optimal primal and dual pair $(\widehat{Y};\widehat{\Lambda})$ of Model
	\cref{formula5}.
The sufficient conditions can be further simplified by  \cref{lem:sufficient_two1,lem:sufficient_two2}. Before further relaxation of the conditions, we introduce some notations for simplicity. Here we define
\begin{equation}
\label{eqn:notation_def_two}
	\left\{
	\begin{array}{ll}
	\epsilon_i=\frac{8m_{1-i}(m_i-1)+4m_i^2}{mm_i^2}\\
	\mu_{pq}=B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq}\\
	\tau_q=\frac{1}{m_0m_1}\sum_{i\in\mathcal{P}^{(1)}}B_{iq}\\
	\rho=\frac{1}{m_0m_1}\sum_{i\in\mathcal{P}^{(1)}}\gamma_{i}
	\end{array}
	\right.
\end{equation}
	where $1\leq p \leq {m\choose 2}$ and $1\leq q\leq n$.
	
\begin{lemma}
\label{lem:sufficient_two1}
Denote $\mathcal{Q}=\{q|\tau_q=0, 1\leq q \leq n\}$. 
	Suppose there exist $c,r\in \mathbb{R}^+$ such that
	\begin{equation}
	\label{eqn:ec_two}
	|\tau_q|>\max_{p\in \mathcal{P}^{(1)}}\left|\frac{mc}{2}(\rho-\gamma_p)\right|,
	\end{equation}
	and
	\begin{equation}
	\label{eqn:cond_two102}
	\frac{2|\tau_q|}{m\rho}>c,
	\end{equation}
	for any $q\not\in\mathcal{Q}$.
Then there exist proper $\widehat\Lambda_{pq}$ ($p\in \mathcal{P}^{(1)},\ 1\leq q\leq n$) to  meet the condition \cref{eqn:cond_two10,eqn:cond_two11}.
\end{lemma} 
\begin{proof}
Since the variable $\vec{\textbf{e}}_q$ is a constant independent from $p$, summing both sides of~\eqref{eqn:cond_two11} for $p\in \mathcal{P}^{(1)}$, we have
	\begin{equation}
	\label{eqn:relax3_two}
	\mu_{pq}=\tau_q+\frac{m}{2m_1m_0}\sum_{i\in\mathcal{P}^{(1)}}\widehat{\Lambda}_{iq}-\frac{mc}{2}\left[\frac{1}{m_0m_1}\sum_{i\in\mathcal{P}^{(1)}}\gamma_i \sign(\mu_{iq})-\gamma_{p}\sign(\mu_{pq})\right].
	\end{equation}
	Notice that $\widehat{\Lambda}^T\in\mathcal{D}^\perp$, we have $\sum_{i\in\mathcal{P}^{(1)}}\widehat{\Lambda}_{iq}=0$. Then, the equality \cref{eqn:relax3_two} can be further simplified as
	\begin{equation}
	\label{eqn:relax4_two}
	\mu_{pq}=\tau_q
	-\frac{mc}{2}\left[\frac{1}{m_0m_1}\sum_{i\in\mathcal{P}^{(1)}}\gamma_i \sign(\mu_{iq})-\gamma_{p}\sign(\mu_{pq})\right].
	\end{equation}
	
	When $q\not\in\mathcal{Q}$,
	if there exist $c,r\in \mathbb{R}^+$ such that
	\[
	|\tau_q|>\max_p\left|\frac{mc}{2}(\rho-\gamma_p)\right|,
	\]
it is easy to see that $\sign(\mu_{pq})=\sign(\tau_q),$
	and \cref{eqn:relax4_two} holds with
	\begin{equation}
	\label{eqn:lambdaf1_two}
	\begin{split}
	&\widehat{\Lambda}_{pq}
	=\frac{2}{m}(\tau_q-B_{pq})-c(\rho-\gamma_{p})\sign(\tau_q).\\
	\end{split}
	\end{equation}

If $q\in\mathcal{Q}$, the inequality~\eqref{eqn:relax4_two} holds by choosing
	\begin{equation}\label{eqn:lambdaf0_two}
	\widehat{\Lambda}_{pq}=-\frac{2}{m}B_{pq}.
	\end{equation}
Therefore, Whenever $\tau_q=0$ or not, $\widehat{\Lambda}_{pq}$ can be written in the form of \cref{eqn:lambdaf1_two}.

Substituting \cref{eqn:lambdaf1_two} into \cref{eqn:cond_two11}, we will have
	\[
	\vec{\mathbf{e}}_q=\tau_q-\frac{mc\rho}{2} \sign(\tau_q),
	\]
	which is independent from index $p$. In other words, the inequality \cref{eqn:ec_two} implies \cref{eqn:cond_two11}.
	
	Secondly, provided that the inequality~\eqref{eqn:ec_two} holds true, we have
	\begin{equation}
	\label{eqn:lambdaf_two}
	\begin{split}
	\mu_{pq}
	=\tau_q-\frac{mc}{2}(\rho-\gamma_{p}){\sign{(\tau_q)}}.
	\end{split}
	\end{equation}
	Then, replacing the term $\mu_{pq}$ in \cref{eqn:cond_two10} by \cref{eqn:lambdaf_two} gives
	\[
	c\gamma_p\leq \frac{2}{m}\left|\tau_q\\
	-\frac{mc}{2}(\rho
	-\gamma_{p})\sign{(\tau_q)}\right|,
	\]
	for any $p\in \mathcal{P}^{(1)}$ and $q\in \mathcal{Q}$.
	
	If 
	\[
	\frac{2|\tau_q|}{m\rho}>c,
	\]
	we have 
	\[
	c\gamma_p\leq\frac{2}{m}|\tau_q|+c\gamma_p-c\rho
	\leq \frac{2}{m}\left||\tau_q|-\frac{mc}{2}(\rho-\gamma_p)\right|
	= \frac{2}{m}\left|\tau_q-\frac{mc}{2}(\rho-\gamma_{p})\sign{(\tau_q)}\right|.
\]
Thus \cref{eqn:ec_two,eqn:cond_two102} imply \cref{eqn:cond_two10,eqn:cond_two11}.
\end{proof}
\begin{lemma}
\label{lem:sufficient_two2}
Assume $\{\widehat{\Lambda}_{pq}\}_{p\in\mathcal{P}^{(1)},1\leq q\leq n}$ satisfies \cref{eqn:cond_two10,eqn:cond_two11}. If
\begin{equation}
	\label{eqn:relaxc2_two}
	\begin{split}
	&\max_{0\leq i\leq 1}\left[{{\epsilon_i}\dia(\mathcal{S}^{(i)})}+\frac{4c m_{1-i}}{m_i}\max_{j\in\mathcal{P}^{(1)}}(\gamma_j)\right]<c\gamma_p,
	\end{split}
	\end{equation}
	for any $p\in \mathcal{P}^{(0)}$. Then there exist $c,r\in\mathbb{R}^+$ and $\widehat{\Lambda}\in\mathcal{D}^\perp$ satisfying Condition \cref{eqn:cond_two2}.
\end{lemma}
\begin{proof}
We will establish that if $\{\widehat{\Lambda}_{pq}\}_{p\in\mathcal{P}^{(1)}}$ satisfies \cref{eqn:cond_two10,eqn:cond_two11}, then there exists $\{\widehat{\Lambda}_{pq}\}_{p\in\mathcal{P}^{(0)}}$,  such that $\widehat{\Lambda}$ belongs to $\mathcal{D}^\perp$, and
		\begin{equation}
		\label{eqn:compare_two}
		\begin{split}
		|\mu_{pq}|\leq& \max\limits_{0\leq i\leq 1}
		\left[\frac{m\epsilon_i\dia(\mathcal{S}^{(i)})}{2}+\frac{2c mm_{1-i}}{m_i}\max_{j\in\mathcal{P}^{(1)}}(\gamma_j)\right]
		\end{split}
		\end{equation}
		for any $ p\in \mathcal{P}^{(0)}$. Combined \cref{eqn:compare_two} with Condition \cref{eqn:relaxc2_two}, we can easily get the conclusion. 
		
		Now we focus on constructing $\hat{\Lambda}\in \mathcal{D}^\perp$ to meet \cref{eqn:compare_two}.
		
		Since $Y\in \mathcal{D}$ if and only if $HY=0$, $\mathcal{D}^\perp$ is exactly the row space of $H$, where $H=(D^{m-1},I)$. Then by direct calculation, ${\widehat{\Lambda}}^T\in \mathcal{D}^\perp$ is equivalent to,
		
		\begin{equation}\label{formula25_two}
		\left( \begin{array}{cc}
		-I_{(m_0-1)\times(m_0-1)},(D^{m_0-1})^T
		\end{array} \right){\hat\Lambda}_{[{\mathcal{P}}_0^{(0)},q]}
		=-\left( \begin{array}{cccc}
		\underset{p\in\mathcal{P}^{(1)}_2}\sum{\hat\Lambda}_{pq},
		\underset{p\in\mathcal{P}^{(1)}_3}\sum{\hat\Lambda}_{pq},
		\dots,
		\underset{p\in\mathcal{P}^{(1)}_{m_0}}\sum{\hat\Lambda}_{pq}
		\end{array} \right)^T
		\end{equation}\\
		and
		\begin{equation}
		\label{formula26_two}
		(D^{m_1})^T{\widehat{\Lambda}}_{[{\mathcal{P}}_1^{(0)},q]}=\sum_{j=1}^{m_0}{\widehat{\Lambda}}_{[{\mathcal{P}}^{(1)}_j,q]},
		\end{equation}
where
\[
{\mathcal{P}}^{(0)}_j=\{(k-1)(m-1)+(l-k)\ |\ k,l\in \mathcal{I}^{(j)}\ with\ k<l\}
\] 
and
\[
{\mathcal{P}}^{(1)}_j=\{(j-1)(m-1)+(i-j)\ |\ i\in \mathcal{I}^{(1)}\}
\] is the subset of $\mathcal{P}^{(1)}$, with $\cup_{l=1}^{m_0}\mathcal{P}^{(1)}_l=\mathcal{P}^{(1)}$. ${\widehat{\Lambda}}_{[{\mathcal{P}}_i^{(j)},q]}$ denotes the column vector whose elements are $\{\widehat{\Lambda}_{pq}\}_{p\in \mathcal{P}_i^{(j)}}$.
		The summation of all elements in the left side of  \cref{formula26_two} is zero, so there exists $\widehat{\Lambda}$ satisfying \cref{formula25_two} and \cref{formula26_two} only if $\sum_{p\in\mathcal{P}^{(1)}}\hat{\Lambda}_{pq}=0$.
		
		For $p\in\mathcal{P}^{(1)}$, by conditions \cref{eqn:cond_two10,eqn:cond_two11}, we have
		\[
	\widehat{\Lambda}_{pq}=\frac{2}{m}\tau_q-\frac{2}{m}B_{pq}-{c}(\rho-\gamma_{p}){\sign(\tau_q)}.
		\]
		Then
		\begin{eqnarray*}
		\frac{m}{2}{\sum_{p\in{\mathcal{P}}_t^{(1)}}\widehat{\Lambda}_{pq}}
		&=&\left({m_1}\tau_q-\sum_{p\in {\mathcal{P}}_t^{(1)}}B_{pq}\right)-\frac{mc}{2}\left(m_1\rho-\sum_{p\in\mathcal{P}^{(1)}_t}\gamma_p\right){\sign(\tau_q)}\\
		&=&-\frac{mcm_1}{2}\left(\rho-\frac{1}{m_1}\sum_{p\in\mathcal{P}^{(1)}_t}\gamma_p\right){\sign(\tau_q)}+\left(\frac{m_1}{m_0}\sum_{i\in\mathcal{I}^{(0)}}A_{iq}-m_1A_{tq}\right).
		\end{eqnarray*}
Obviously, $\sum_{t=1}^{m_0}{\sum_{p\in{\mathcal{P}}_t^{(1)}}\widehat{\Lambda}_{pq}}=0$ and
		\[
		\left\|\frac{m}{2}{\widehat{\Lambda}}_{[{\mathcal{P}}_t^{(1)},q]}\right\|_\infty\leq \frac{m_1(m_0-1)}{m_0}\dia(\mathcal{S}^{(0)})+{cm}{m_1}\max_{p\in \mathcal{P}^{(1)}}(\gamma_p)
		\]
		for any $t\in \mathcal{I}^{(0)}$.
		
	Considering the constraint 
	\begin{equation}
	\label{eqn:restrictConst}
	(D^{m_0})^T{\widehat{\Lambda}}_{[{\mathcal{P}}_0^{(0)},q]}=-\left( \begin{array}{cccc}
		\underset{p\in\mathcal{P}^{(1)}_1}\sum{\hat\Lambda}_{pq},
		\underset{p\in\mathcal{P}^{(1)}_2}\sum{\hat\Lambda}_{pq},
		\dots,
		\underset{p\in\mathcal{P}^{(1)}_{m_0}}\sum{\hat\Lambda}_{pq}
		\end{array} \right)^T,	\end{equation}
	we can see that  \cref{formula25_two} is the sub-constraint of \cref{eqn:restrictConst}.	Therefore, we need to find proper $\widehat\Lambda$ obeying \cref{eqn:restrictConst,formula26_two}.
	
	By \cite[Lemma 3]{zhu2014convex}, given $C_n\in \mathbb{R}^n$, i.e. $C_n=(c_1,c_2,\dots,c_n)^T$ such that  $\sum_{i=1}^n c_i=0$, there exists $X\in \mathbb{R}^{C_n^2}$ with $\|X\|_{\infty}\leq\frac{2}{n}M$ and $(D^n)^TX=C_n$, where  $\|C_n\|_{\infty}\leq M$. 
So there exist $\widehat{\Lambda}_{pq}(\ p\in\mathcal{P}^{(0)}_0)$ satisfying \eqref{formula25_two} and
		\[
		\left|\frac{m}{2}{\widehat{\Lambda}}_{pq}\right|\leq
		\frac{2m_1(m_0-1)}{m_0^2}\dia(\mathcal{S}^{(0)})+\frac{2cmm_1}{m_0}\max_{i\in \mathcal{P}^{(1)}}(\gamma_i).
		\]
		Furthermore, we have
		\begin{equation}
		\label{eqn:I0constraint}
		\left|B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq}\right|\leq
		\frac{4m_1(m_0-1)+2m_0^2}{m_0^2}\dia(\mathcal{S}^{(0)})+\frac{2c mm_1}{m_0}\max_{i\in\mathcal{P}^{(1)}}(\gamma_i),
		\end{equation}
for $p\in \mathcal{P}_0^{(0)}$.

By the symmetry of $\widehat{\Lambda}_{pq}(p\in\mathcal{P}^{(0)}_0)$ and $\widehat{\Lambda}_{pq}(p\in\mathcal{P}^{(0)}_1)$, there exist $\widehat{\Lambda}_{pq}(p\in\mathcal{P}^{(0)}_1)$  satisfying \eqref{formula26_two}, and
		\begin{equation}
		\label{eqn:I1constraint}
		\left|B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq}\right|\leq
		\frac{4m_0(m_1-1)+2m_1^2}{m_1^2}\dia(\mathcal{S}^{(1)})
		+\frac{2c mm_0}{m_1}\max_{i\in\mathcal{P}^{(1)}}(\gamma_i),
		\end{equation}
for $p\in\mathcal{P}_1^{(0)}$.

Therefore, \cref{eqn:I0constraint,eqn:I1constraint} meets the condition \cref{eqn:compare_two}.
\end{proof}

Now, we begin to prove \cref{theorem_twobody}.
\begin{proof}[Proof of \cref{theorem_twobody}]
If there exist $c$ and $r$ such that they can guarantee the conditions \cref{eqn:ec_two,eqn:cond_two102,eqn:relaxc2_two} in \cref{lem:sufficient_two1,lem:sufficient_two2}, we have optimal solution satisfying exact clustering property. 

Here the condition \cref{eqn:relaxc2_two} is equivalent to 
\begin{equation}
	\label{eqn:condf3_two}
	\gamma_p-\frac{4 (m-m_i)}{m_i}\max_{j\in\mathcal{P}^{(1)}}(\gamma_j)>0
	\end{equation}
	and
	\begin{equation}
	\label{eqn:condf4_two}
	\frac{\epsilon_i\dia(\mathcal{S}^{(i)})}{\gamma_p -4\frac{(m-m_i)}{m_i}\max_{j\in\mathcal{P}^{(1)}}(\gamma_j)}<c,
	\end{equation}
for any $p\in\mathcal{P}^{(0)}$ and $i\in \{0,1\}$.
	Recall that $\gamma_i$ is defined as 
	\[
	\gamma_i=\exp({-r\|(DA)_i\|_2^2}).
	\]
	Then the separation property 
	\[
	\dist(\mathcal{S}^{(0)},\mathcal{S}^{(1)})>\max\{\dia(\mathcal{S}^{(0)}), \dia(\mathcal{S}^{(1)})\}
	\]
	implies that
	\[
	\lim\limits_{r\rightarrow+\infty}\max\limits_{i\in\mathcal{P}^{(1)}}(\gamma_i)=0 ~\text{and}~\lim\limits_{r\rightarrow+\infty}\frac{\min_{p'\in \mathcal{P}^{(1)}}\gamma_{p'}}{\max_{p\in \mathcal{P}^{(0)}}\gamma_{p}}=0.\]
If there exist $c,r$ such that
\begin{equation}
	\label{eqn:existc1_two}
	\frac{|\tau_q|}{\epsilon_i\dia(\mathcal{S}^{(i)})}>\frac{\max_{p'\in \mathcal{P}^{(1)}}|\frac{m}{2}(\rho-\gamma_{p'})|}{\gamma_p-\frac{4m_{1-i}}{m_i}\max_{i\in\mathcal{P}^{(1)}}(\gamma_i)}
	\end{equation}
for any $q\not\in\mathcal{Q}$ and $p\in \mathcal{P}^{(0)}$, then the inequalities \cref{eqn:ec_two} and \cref{eqn:condf4_two} hold true.
When taking $r\rightarrow+\infty$ on both sides of \cref{eqn:existc1_two}, the left hand side converges to  a finite constant and  the right hand side goes to  zero. 

By similar arguments, there exists a positive constant $r_0$ such that \cref{eqn:ec_two,eqn:cond_two102,eqn:condf3_two,eqn:condf4_two} hold true for any $r>r_0$.
\end{proof}

\subsection{Proof of \cref{theorem1}}
\label{sec:prf of three-cluster}
 The sufficient condition for exact clustering is similar as $2$-cluster case.
\begin{theorem}[sufficient condition for $K$-cluster]
\label{thm:suf_three}
 Assume $c,r\in \mathbb{R}^+$ and $\widehat{\Lambda}^T\in \mathcal{D}^\perp$.   $\vec{\textbf{e}}^{k,l}(0\leq k<l\leq K-1)$ are nonzero column vectors in $\mathbb{R}^n$. $\mathcal{P}^{(0)}$ and $\mathcal{P}^{(k,l)}$ are defined in \cref{eqn:P0} and \cref{eqn:Pkl}. Suppose for $p\in\mathcal{P}^{(k,l)}(0\leq k<l\leq K-1)$, $\widehat\Lambda_{pq}$ satisfies	
	\begin{subequations}
	\begin{align}
	&c\gamma_{p}\leq \frac{2}{m}|B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq}|,\label{eqn:cond10}\\
	&(B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq})-\frac{mc \gamma_{p}}{2}\sign(B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq})=\vec{\textbf{e}}^{k,l}_q,\label{eqn:cond11}
	\end{align}
	\end{subequations}
		 and for $p\in\mathcal{P}^{(0)}$, we have
		\begin{equation}
		\label{eqn:cond2}
		c\gamma_p>\frac{2}{m}|B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq}|.
		\end{equation}
		Besides, $\vec{\textbf{e}}$ meet the condition
		\begin{equation}
	\label{eqn:cond3}
		\vec{\textbf{e}}^{k,l}_q+\vec{\textbf{e}}^{l,m}_q=\vec{\textbf{e}}^{k,m}_q
		\end{equation}
		for all $0\leq k<l<m\leq K-1$.
		
Then $\widehat{\Lambda}$ is the optimal dual variable in \cref{eqn:dual}, and $\widehat{Y}$ can be derived respectively. Together with the fact that $\widehat{Y}=D\widehat{X}$, $\hat{X}$ satisfies the exact clustering property.
\end{theorem}

The condition \cref{eqn:cond3} is not seen in $2$-cluster case, which leads to different primal dual $(\widehat{Y},\widehat{\Lambda})$ construction for $K\geq 3$. 
For simplicity of notation, we only consider $K=3$ in \cref{theorem1} and the general case can be derived by the same method.

When $K=3$, under the condition in \cref{thm:suf_three}, we have 
\[\vec{\textbf{e}}^{0,1}+\vec{\textbf{e}}^{1,2}=\vec{\textbf{e}}^{0,2},\] and  $\widehat{X}$ has exact clustering property with
	\[\widehat{X}_{i}=
	\left\{ \begin{array}{l}
	\frac{m_1}{m}\vec{\textbf{e}}^{0,1}+\frac{m_2}{m}\vec{\textbf{e}}^{0,2}, \quad i\in\mathcal{I}^{(0)},\\
	\frac{m_1}{m}\vec{\textbf{e}}^{0,1}+\frac{m_2}{m}\vec{\textbf{e}}^{0,2}-\vec{\textbf{e}}^{0,1}, \quad i\in\mathcal{I}^{(1)},\\
	\frac{m_1}{m}\vec{\textbf{e}}^{0,1}+\frac{m_2}{m}\vec{\textbf{e}}^{0,2}-\vec{\textbf{e}}^{0,2}, \quad i\in\mathcal{I}^{(2)}.
	\end{array} \right.
	\]
Here we define
\[
	\left\{
	\begin{array}{ll}
	\epsilon_i=\frac{8(m-m_i)(m_i-1)+4m_i^2}{mm_i^2}\\
	\mu_{pq}=B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq}\\
	\tau^{k,l}_q=\frac{1}{m_km_l}\sum_{i\in\mathcal{P}^{(k,l)}}B_{iq}\\
	\rho^{k,l}=\frac{1}{m_km_l}\sum_{i\in\mathcal{P}^{(k,l)}}\gamma_{i}
	\end{array}
	\right.
	\]
	where $1\leq p \leq {m\choose 2}, 1\leq q\leq n, 0\leq i\leq 2, 0\leq k<l\leq 2
	$.
	
	For $p\in \mathcal{P}^{(1)}$ and $1\leq q\leq n$, construct specific $\widehat\Lambda_{pq}$ as 
	\begin{equation}
	\label{eqn:mu_pq}
	\frac{m}{2}\widehat\Lambda_{pq}=
	\left\{ \begin{array}{l}
	-B_{pq}+\tau^{0,1}_q+\frac{mc}{2}(\gamma_{p}-\rho^{0,1})\sign(\tau_q^{0,1})+m_2H_q,
	\quad \mbox{if}\ p\in\mathcal{P}^{(0,1)},\\
	-B_{pq}+\tau^{1,2}_q+\frac{mc}{2}(\gamma_{p}-\rho^{1,2})\sign(\tau_q^{1,2})+m_0H_q,
	\quad \mbox{if}\ p\in\mathcal{P}^{(1,2)},\\
	-B_{pq}+\tau^{0,2}_q+\frac{mc}{2}(\gamma_{p}-\rho^{0,2})\sign(\tau_q^{0,2})-m_1H_q,
	\quad \mbox{if}\ p\in\mathcal{P}^{(0,2)},\\
	\end{array} \right.
	\end{equation}
	where
	\[
	H_q=\frac{c}{2}\left(\rho^{0,1}\sign(\tau_q^{0,1})+\rho^{1,2}\sign(\tau_q^{1,2})-\rho^{0,2}\sign(\tau_q^{0,2})\right).
	\]

\cref{lem:suf_three1,lem:sufficient_three2} show proper sufficient condition of $\widehat{\Lambda}_{pq}$ to meet the Conditions \cref{eqn:cond10,eqn:cond11,eqn:cond2,eqn:cond3} in \cref{thm:suf_three}.
\begin{lemma}
\label{lem:suf_three1}
For each pair of $(k,l)$, suppose there exist $c,r\in \mathbb{R}^+$ such that
\begin{equation}
	\label{eq:eqn141}
	\left|\tau_q^{k,l}\right|-\frac{3mc}{2}\max_{i\in \mathcal{P}^{(1)}}\gamma_i>\max_{p\in \mathcal{P}^{(k,l)}}\frac{mc}{2}\left|\rho^{k,l}-\gamma_p\right|
	\end{equation}
	and
	\begin{equation}
	\label{eq:eqn151}
	\left|\tau_q^{k,l}\right|-\frac{3mc}{2}\max_{i\in \mathcal{P}^{(1)}}\gamma_i>\frac{mc}{2}\rho^{k,l}
	\end{equation}
	For $p\in \mathcal{P}^{(1)}$, $\widehat\Lambda_{pq}$ is defined in \cref{eqn:mu_pq}. Then $\widehat\Lambda$ meet the conditions \cref{eqn:cond10,eqn:cond11,eqn:cond3}. 
	\end{lemma}
	\begin{proof}
	By the definition of $H_q$, we have 
	\[
	|H_q|\leq \frac{3c}{2}\max_{i\in \mathcal{P}^{(1)}}\gamma_i.
	\]
	Combining with the condition \cref{eq:eqn141}, we get 
	\begin{equation}
	\label{eqn:inequ14}
	|\tau_q^{k,l}|>\max_{p\in \mathcal{P}^{(k,l)}}\frac{mc}{2}\left|\rho^{k,l}-\gamma_{p}\right|+m|H_q|.
	\end{equation}
	Then $\sign(\mu_{pq})=\sign(\tau^{k,l}_q)$ for $p\in \mathcal{P}^{(k,l)}$.

Secondly, provided that \cref{eq:eqn141,eq:eqn151} holding true, we obtain
\begin{equation}
	\label{conditionI1}
	\left|\tau^{0,1}_q+\frac{mc}{2}(\gamma_{p}-\rho^{0,1})\sign(\tau_q^{0,1})+m_2H_q\right|\geq \frac{m}{2}c\gamma_p,\quad p\in \mathcal{P}^{(0,1)},
	\end{equation}
	\begin{equation}
	\label{conditionI2}
	\left|\tau^{1,2}_q+\frac{mc}{2}(\gamma_{p}-\rho^{1,2})\sign(\tau_q^{1,2})+m_0H_q\right|\geq \frac{m}{2}c\gamma_p,\quad p\in \mathcal{P}^{(1,2)},
	\end{equation}
and\begin{equation}
	\label{conditionI3}
	\left|\tau^{0,2}_q+\frac{mc}{2}(\gamma_{p}-\rho^{0,2})\sign(\tau_q^{0,2})-m_1H_q\right|\geq \frac{m}{2}c\gamma_p, \quad p\in \mathcal{P}^{(0,2)}.
	\end{equation}
	Thus the inequality \eqref{eqn:cond10} holds true, and
	\[
	\left\{
	\begin{array}{ll}
	\vec{\mathbf{e}}_q^{0,1}=\tau^{0,1}_q-\frac{mc}{2}\rho^{0,1}\sign(\tau_q^{0,1})+m_2H_q,\\
	\vec{\mathbf{e}}_q^{1,2}=\tau^{1,2}_q-\frac{mc}{2}\rho^{1,2}\sign(\tau_q^{1,2})+m_0H_q,\\
	\vec{\mathbf{e}}_q^{0,2}=\tau^{0,2}_q-\frac{mc}{2}\rho^{0,2}\sign(\tau_q^{0,2})-m_1H_q,
	\end{array}
	\right.
	\]
	to get \cref{eqn:cond11,eqn:cond3}.
	\end{proof}
	
	\begin{lemma}
\label{lem:sufficient_three2}
Assume $\{\widehat{\Lambda}_{pq}\}_{p\in\mathcal{P}^{(k,l)},1\leq q\leq n}$ defined in \cref{eqn:mu_pq} satisfies \cref{eqn:cond10,eqn:cond11,eqn:cond3}. If
\begin{equation}
	\label{eqn:relaxc2}
	\begin{split}
	&\max_{0\leq i\leq 2}\left[{{\epsilon_i}\dia(\mathcal{S}^{(i)})}+\frac{4c (m-m_i)}{m_i}\max_{j\in\mathcal{P}^{(1)}}(\gamma_j)\right]<c\gamma_p,
	\end{split}
	\end{equation}
	for all $p\in \mathcal{P}^{(0)}$. Then there exist $c,r\in\mathbb{R}^+$ and $\widehat{\Lambda}\in\mathcal{D}^\perp$ satisfying Condition \cref{eqn:cond2}.
\end{lemma}
\begin{proof}
We show that, if $\{\widehat{\Lambda}_{pq}\}_{p\in\mathcal{P}^{(k,l)}}$ satisfies \cref{eqn:cond10,eqn:cond11,eqn:cond3}, then there exists $\{\widehat{\Lambda}_{pq}\}_{p\in\mathcal{P}^{(0)}}$,  such that $\widehat{\Lambda}$ belongs to $\mathcal{D}^\perp$, and
		\begin{equation}
		\label{eqn:compare}
		\begin{split}
		|\mu_{pq}|\leq& \max\limits_{0\leq i\leq 2}
		\left[\frac{m\epsilon_i\dia(\mathcal{S}^{(i)})}{2}+\frac{2c m(m-m_i)}{m_i}\max_{j\in\mathcal{P}^{(1)}}(\gamma_j)\right]
		\end{split}
		\end{equation}
		for any $ p\in \mathcal{P}^{(0)}$. Combined \cref{eqn:compare} with Condition \cref{eqn:relaxc2}, we can  get the conclusion. 

By direct calculation, ${\widehat{\Lambda}}^T\in \mathcal{D}^\perp$ is equivalent to,
		
		\begin{equation}\label{formula25}
		\left( \begin{array}{cc}
		-I_{(m_0-1)\times(m_0-1)},(D^{m_0-1})^T
		\end{array} \right){\Lambda}_{[{\mathcal{P}}_0^{(0)},q]}
		=-\left( \begin{array}{cccc}
		\underset{p\in\mathcal{P}^{(0,1)}_2\cup\mathcal{P}^{(0,2)}_2}\sum{\Lambda}_{pq},
		\dots,
		\underset{p\in\mathcal{P}^{(0,1)}_{m_0}\cup\mathcal{P}^{(0,2)}_{m_0}}\sum{\Lambda}_{pq}
		\end{array} \right)^T
		\end{equation}
		\begin{equation}
		\label{formula261}
		(D^{m_1})^T{\widehat{\Lambda}}_{[{\mathcal{P}}_1^{(0)},q]}\\
		=-\left(\begin{array}{cccc}
		\underset{p\in\mathcal{P}^{(1,2)}_{m_0+1}}\sum{\Lambda}_{pq},
		\underset{p\in\mathcal{P}^{(1,2)}_{m_0+2}}\sum{\Lambda}_{pq},
		\dots,
		\underset{p\in\mathcal{P}^{(1,2)}_{m_0+m_1}}\sum{\Lambda}_{pq}
		\end{array}\right)^T
		+\sum_{j=1}^{m_0}{\widehat{\Lambda}}_{[{\mathcal{P}}^{(0,1)}_j,q]}
		\end{equation}
		\begin{equation}
		\label{formula26}
		(D^{m_2})^T{\widehat{\Lambda}}_{[{\mathcal{P}}_2^{(0)},q]}=\sum_{j=1}^{m_0}{\widehat{\Lambda}}_{[{\mathcal{P}}^{(0,2)}_j,q]}+\sum_{j=m_0+1}^{m_0+m_1}{\widehat{\Lambda}}_{[{\mathcal{P}}^{(1,2)}_j,q]},
		\end{equation}
where \[
\mathcal{P}^{(0)}_k=\{(i-1)(m-1)+(j-i)\ |\ i<j,\  i,j\in\mathcal{I}^{(k)}\},
\]
and
\[{\mathcal{P}}^{(k,l)}_j=\{(j-1)(m-1)+(i-j)\ |\ i\in \mathcal{I}^{(l)}\}\] with $j\in \mathcal{I}^{(k)}$, and ${\widehat{\Lambda}}_{[{\mathcal{P}}_j^{(k,l)},q]}$ denotes the column vector whose elements are $\{\widehat{\Lambda}_{pq}\}_{p\in \mathcal{P}_j^{(k,l)}}$.

Consider the construction of $\widehat{\Lambda}_{[{\mathcal{P}}_2^{(0)},q]}$. Since $\{\widehat{\Lambda}_{pq}\}_{p\in\mathcal{P}^{(k,l)}}$ is defined in \cref{eqn:mu_pq}, we have the RHS of \eqref{formula26} equalling to zero by direct calculation.

Besides,
\begin{align}	
&\left\|\frac{m}{2}\left(\sum_{j=1}^{m_0}{\widehat{\Lambda}}_{[{\mathcal{P}}^{(0,2)}_j,q]}+\sum_{j=m_0+1}^{m_0+m_1}{\widehat{\Lambda}}_{[{\mathcal{P}}^{(1,2)}_j,q]}\right)\right\|_\infty\nonumber\\
		&\leq \frac{(m-m_2)(m_2-1)}{m_2}\dia(\mathcal{S}^{(2)})
		+cm(m-m_2)\max_{p\in \mathcal{P}^{(1)}}(\gamma_p).\nonumber
		\end{align}
Applying  \cite[Lemma 3]{zhu2014convex}, there exist $\widehat{\Lambda}_{pq} (p\in\mathcal{P}^{(0)}_2)$ satisfying
		\[
		\left|\frac{m}{2}{\widehat{\Lambda}}_{pq}\right|\leq
		\frac{2(m-m_2)(m_2-1)}{m_2^2}\dia(\mathcal{S}^{(2)})
		+\frac{2cm(m-m_2)}{m_2}\max_{i\in \mathcal{P}^{(1)}}(\gamma_i).
		\]
		Furthermore,
		\[
		\left|B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq}\right|\leq
		\frac{4(m-m_2)(m_2-1)+2m_2^2}{m_2^2}\dia(\mathcal{S}^{(2)})
		+\frac{2c m(m-m_2)}{m_0}\max_{i\in\mathcal{P}^{(1)}}(\gamma_i),\ p\in \mathcal{P}_2^{(0)},
		\]
		By the same analysis, there exist $\widehat{\Lambda}_{pq}(p\in\mathcal{P}^{(0)}_k)$  satisfying \eqref{formula25}, \eqref{formula261} and \eqref{formula26} with
		\[
		\left|B_{pq}+\frac{m}{2}\widehat{\Lambda}_{pq}\right|\leq
		\frac{4(m-m_k)(m_k-1)+2m_k^2}{m_k^2}\dia(\mathcal{S}^{(k)})
		+\frac{2c m(m-m_k)}{m_k}\max_{i\in\mathcal{P}^{(1)}}(\gamma_i),\ p\in\mathcal{P}_k^{(0)}.
		\]
		Therefore, the condition \cref{eqn:compare} is satisfied.
\end{proof}

Now, we begin to prove \cref{theorem1}.
\begin{proof}[Proof of \cref{theorem1}]
If there exist $c$ and $r$ such that they can guarantee the conditions \cref{eq:eqn141,eq:eqn151,eqn:relaxc2} in \cref{lem:suf_three1,lem:sufficient_three2}, we have optimal solution satisfying exact clustering property. 

Condition \cref{eqn:relaxc2} is equivalent to 
\begin{equation}
	\label{eqn:condf3}
	\gamma_p-\frac{4 (m-m_i)}{m_i}\max_{j\in\mathcal{P}^{(1)}}(\gamma_j)>0,
	\end{equation}
	and
	\begin{equation}
	\label{eqn:condf4}
	\frac{\epsilon_i\dia(\mathcal{S}^{(i)})}{\gamma_p -4 \frac{m-m_i}{m_i}\max_{j\in\mathcal{P}^{(1)}}(\gamma_j)}<c,
	\end{equation}
	for any $p\in\mathcal{P}^{(0)}$ and $0\leq i\leq 2$.

There exist $c$ and $r$ such that the condition \cref{eq:eqn141}  and \cref{eqn:condf4} hold true  if and only if
	\begin{equation}
	\label{eqn:existc1}
	\frac{|\tau_q^{k,l}|}{\epsilon_i\dia(\mathcal{S}^{(i)})}>\frac{\frac{m}{2}\left[\max_{p'\in \mathcal{P}^{(k,l)}}|(\rho^{k,l}-\gamma_{p'})|+3\max_{i\in \mathcal{P}^{(1)}}\gamma_i\right]}{\gamma_p-\frac{4(m-m_i)}{m_i}\max_{i\in\mathcal{P}^{(1)}}(\gamma_i)},
	\end{equation}
	for any $1\leq q\leq n$, $0\leq i\leq 2$, $0\leq k<l\leq 2$, and $p\in\mathcal{P}^{(0)}$.
	
	
	Since $
	\gamma_i=\exp({-r\|(DA)_i\|_2^2}),
	$
	the separation property \cref{eqn:sep} implies that
	$$\lim\limits_{r\rightarrow+\infty}\max\limits_{i\in\mathcal{P}^{(1)}}(\gamma_i)=0 ~\text{and}~\lim\limits_{r\rightarrow+\infty}\frac{\min_{p'\in \mathcal{P}^{(1)}}\gamma_{p'}}{\max_{p\in \mathcal{P}^{(0)}}\gamma_{p}}=0.$$
	Besides, by the assumption of \cref{theorem1}, the centres of each cluster are distinct in all dimensions. Therefore, when taking $r\rightarrow+\infty$ on both sides of \cref{eqn:existc1}, the left side converges to  a finite positive constant and  the right hand side goes to  zero.
	Similarly, the inequalities \cref{eq:eqn141,eq:eqn151,eqn:condf3,eqn:condf4} can also hold true when $r\rightarrow +\infty$.  Therefore, there exists a positive constant $r_0$ such that \cref{eq:eqn141,eq:eqn151,eqn:condf3,eqn:condf4} hold for any $r>r_0$.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{The proof of \cref{thm:GaussianMixture}}
In order to prove \cref{thm:GaussianMixture}, we introduce some technical lemmas.
\begin{lemma}[\cite{LM2000}]
\label{main lemma}Let $(X_{1},...,X_{m})$ be i.i.d. Gaussian variables,
with mean $0$ and variance $1$. Let $\lambda=[\lambda_{1},...,\lambda_{m}]$ be a non-negative vector. Denote $Y=\sum_{i=1}^{m}\lambda_{i}X_{i}^{2}$. Then  for any $t>0$, we have
\[
\mathbb{P}(Y\geq\|\lambda\|_{1}+2\|\lambda\|_{2}\sqrt{t}+2\|\lambda\|_{\infty}t)\leq\exp(-t),
\]
\[
\mathbb{P}(Y\leq\|\lambda\|_{1}-2\|\lambda\|_{2}\sqrt{t})\leq\exp(-t).
\]
\end{lemma}
\begin{lemma}
\label{prop: Main proposition}Let $x$ sampled from $\mathcal{N}(\mu,\Sigma)$,
where $\Sigma\in\mathbb{R}^{n\times n}$ is the covariance matrix.
If $\mu=0$, then
\begin{equation}
\mathbb{P}(\|x\|_{2}^{2}\geq\mbox{\text{Tr}}(\Sigma)+2\|\Sigma\|_{F}\sqrt{t}+2\|\Sigma\|t)\leq\exp(-t),\qquad\text{for}\ t>0.\label{eq: upper bound inequality}
\end{equation}
 For arbitrary $\mu$, we get
\begin{equation}
\mathbb{P}\left(\|x\|_{2}^{2}\leq\|\mu\|_{2}^{2}+\text{Tr(\ensuremath{\Sigma})}-(2\|\Sigma\|_{F}+2\|\Sigma\|^{\frac{1}{2}}\|\mu\|_{2})\sqrt{t}\right)\leq2\exp(-t)\qquad\text{for}\ t>0.\label{eq: lower bound inequality}
\end{equation}
\end{lemma}
\begin{proof}
The singular value decomposition of $\Sigma$ is $U\varLambda U^{*}$,
where $U\in\mathbb{R}^{n\times n}$ is an unitary matrix and $\Lambda$
is a positive semi-definite diagonal matrix. Denote $\Lambda^{\frac{1}{2}}$
as the squared root of $\Lambda$. If $y\sim\mathcal{N}(0,I)$, 
$\|\Lambda^{\frac{1}{2}}y\|_{2}$ and $\|x\|_{2}$ have the same distribution
when $\mu=0$. Then applying Lemma \ref{main lemma} with $\lambda_{i}=\Lambda_{i}$,
where $\Lambda_{i}$ is the $i$th element in the diagonal of $\Lambda$, we can get (\ref{eq: upper bound inequality}). 

Now we prove inequality (\ref{eq: lower bound inequality}) when $\mu\neq0$. Since $U^{*}$ is unitary,
$\|x\|_{2}^{2}$ has the same distribution with $\|U^{*}x\|_{2}^{2}$. Then $U^{*}x\sim\mathcal{N}(\tilde{\mu},\Lambda)$,
where $\tilde{\mu}=U^{*}\mu$. Denote $z=\Lambda^{\frac{1}{2}}y+\tilde{\mu}$,
where $y\sim\mathcal{N}(0,I)$. Then $z$ has the same distribution
as $U^{*}x$. We can see that $\|z\|_{2}^{2}=\|\Lambda^{\frac{1}{2}}y\|_{2}^{2}+2\langle\tilde{\mu},\Lambda^{\frac{1}{2}}y\rangle+\|\tilde{\mu}\|_{2}^{2}$. By \cref{main lemma}, we obtain that 
\begin{equation}
\label{eqn:inequ1_appendix}
\mathbb{P}\left(\|\Lambda^{\frac{1}{2}}y\|_{2}^{2}\leq \text{Tr}(\Lambda)-2\|\Lambda\|_{F}\sqrt{t}=\text{Tr}(\Sigma)-2\|\Sigma\|_{F}\sqrt{t}\right)\leq\exp(-t).
\end{equation}


Meanwhile, we get that $\langle \tilde{\mu},\Lambda^{\frac{1}{2}}y\rangle$ is
distributed as $\mathcal{N}(0,\mu^{T}\Sigma\mu)$. Since
\[
\mathbb{P}\left(\left|\frac{\langle\tilde{\mu},\Lambda^{\frac{1}{2}}y\rangle}{\sqrt{\mu^{T}\Sigma\mu}}\right|>t\right)\leq\exp(-t^{2}/2),\quad \text{for}\ t>0
\]
by the tail bound of standard Gaussian distribution, therefore 
\begin{equation}
\label{eqn:inequ2_appendix}
\mathbb{P}\left(\langle\tilde{\mu},\Lambda^{\frac{1}{2}}y\rangle<-2\|\Sigma\|^{\frac{1}{2}}\|\mu\|_{2}\sqrt{t}\right)\leq\mathbb{P}\left(\frac{\langle\tilde{\mu},\Lambda^{\frac{1}{2}}y\rangle}{\sqrt{\mu^{T}\Sigma\mu}}<-2\sqrt{t}\right)\leq\exp(-t),
\end{equation}
for all $t>0$. For arbitrary random variables $X$ and $Y$, we have
\[
\mathbb{P}(X+Y\leq a+b)\leq\mathbb{P}(X\leq a)+\mathbb{P}(Y\leq b).
\]
Combining \cref{eqn:inequ1_appendix,eqn:inequ2_appendix}, we obtain
\[
\mathbb{P}(\|x\|_{2}^{2}\leq\|\mu\|_{2}^{2}+\text{Tr(\ensuremath{\Sigma})}-(2\|\Sigma\|_{F}+2\|\Sigma\|^{\frac{1}{2}}\|\mu\|_{2})\sqrt{t})\leq2\exp(-t)\qquad\text{for}\ t>0.
\]
\end{proof}
Now we begin to prove the theorem.
\begin{proof}[Proof of \cref{thm:GaussianMixture}]
Since the centers $\mu_k$ of gaussian distributions are distinct in each dimension, the mean values of samples inside each cluster are different in each dimension with probability $1$.
In order to have inner-class distance smaller than the inter-class
distance with high probability, we should have 
$
\|A_{i}-A_{j}\|_2>\|A_{k_1}-A_{k_2}\|_2
$
 for all $i\in\mathcal{S}^{(k)}$, $j\in\mathcal{S}^{(l)}$ ($0\leq k<l\leq K-1$) and $k_{1},k_{2}\in\mathcal{S}^{(i)}$($i=0,\cdots,K-1$).
 
 If $i\in\mathcal{S}^{(k)}$, $j\in\mathcal{S}^{(l)}$, we can see that $A_{i}-A_{j}\sim\mathcal{N}(\mu_{k}-\mu_{l},\Sigma_{k}+\Sigma_{l})$. Based on \cref{prop: Main proposition}, for fixed $k$ and $l$, we have
\begin{eqnarray*}
\mathbb{P}\biggl(\exists i\in\mathcal{S}^{(k)},j\in\mathcal{S}^{(l)}\quad  &  & \|A_{i}-A_{j}\|_{2}^{2}\leq\|\mu_{k}-\mu_{l}\|_{2}^{2}+\text{Tr}(\Sigma_{k}+\Sigma_{l})\\
 &  & -(2\|\Sigma_{k}+\Sigma_{l}\|_{F}+2\|\Sigma_{k}+\Sigma_{l}\|^{\frac{1}{2}}\|\mu_{k}-\mu_{l}\|_{2})\sqrt{3\log m}\biggr)\\
 &  & \leq \frac{2 m_km_l}{m^{3}}.
\end{eqnarray*}
Meanwhile, for $k_{1},k_{2}\in\mathcal{S}^{(i)}$($0\leq i\leq K-1$) with $k_1\neq k_2$, we get $A_{k_{1}}-A_{k_{2}}\sim\mathcal{N}(0,2\Sigma_{i})$ and the union bound for all clusters becomes
\begin{eqnarray*}
\mathbb{P}(\exists k_{1},k_{2}\in\mathcal{S}^{(i)}\quad & \|A_{k_{1}}-A_{k_{2}}\|_{2} & \geq\max_{i}(\text{Tr}(\Sigma_{i})+2\|\Sigma_{i}\|_{F}\sqrt{3\log m}+6\|\Sigma_{i}\|\log m))\\
 &  & \leq \frac{\sum_i m_i(m_i-1)}{2m^3}.
\end{eqnarray*}

Based on  the above two inequalities, if for all $0\leq k<l\leq K-1$, 
\begin{equation}
\begin{split}
\|\mu_{k}-\mu_{l}\|_{2}^{2}+\text{Tr}(\Sigma_{k,l}) & -  (2\|\Sigma_{k,l}\|_{F}+2\|\Sigma_{k,l}\|^{\frac{1}{2}}\|\mu_{k}-\mu_{l}\|_{2})\sqrt{3\log m}\\
 &  >\text{\ensuremath{\max}}_{i}(\mbox{\text{Tr}}(\Sigma_{i})+2\|\Sigma_{i}\|_{F}\sqrt{3\log m}+6\|\Sigma_{i}\|\log m),
 \end{split}
\end{equation}
where $\Sigma_{k,l}=\Sigma_{k}+\Sigma_{l}$,  we have $
\|A_{i}-A_{j}\|_2>\|A_{k_1}-A_{k_2}\|_2
$
 for all $i\in\mathcal{S}^{(k)}$, $j\in\mathcal{S}^{(l)}$ ($0\leq k<l\leq K-1$) and $k_{1},k_{2}\in\mathcal{S}^{(i)}$($i=0,\cdots,K-1$) with probability larger than $1-3/m$.
 
 Therefore, if 
 \begin{eqnarray*}
\|\mu_{k}-\mu_{l}\|_2 & > & \|\Sigma_{k,l}\|^{\frac{1}{2}}\sqrt{12\log m}+{(12\log m)}^{1/4}\|\Sigma_{k,l}\|_{F}^{1/2}\\
 &  & +\max_i\sqrt{{\text{Tr}}(\Sigma_{i})+2\|\Sigma_{i}\|_{F}\sqrt{3\log n}+2\|\Sigma_{i}\|3\log m},
\end{eqnarray*}
for all $0\leq k<l\leq K-1$, we have the exact recovery of model \cref{eqn:weightconvex}.
\end{proof}

